Fast Combinatorial Algorithms for Min Max Correlation Clustering

We introduce fast algorithms for correlation clustering with respect to the Min Max objective that provide constant factor approximations on complete graphs. Our algorithms are the first purely combinatorial approximation algorithms for this problem. We construct a novel semi-metric on the set of vertices, which we call the correlation metric, that indicates to our clustering algorithms whether pairs of nodes should be in the same cluster. The paper demonstrates empirically that, compared to prior work, our algorithms sacrifice little in the objective quality to obtain significantly better run-time. Moreover, our algorithms scale to larger networks that are effectively intractable for known algorithms.

==> Correlation Clustering/experiments.tex <==
\section{Experiments} \label{sec: experiments}
In this section, we describe experiments supporting our theoretical results.\footnote{The code for our experiments can be found at https://github.com/hanewman/MinMax-Correlation-Clustering-} We demonstrate:
\begin{itemize}
\item The guarantees of Theorem \ref{thm: apx_thm} are predictive of 
our algorithm's performance on real-world and synthetic datasets. Our algorithm's solution quality is similar to the KMZ algorithm. 
\item The fractional cost of the correlation metric is similar to the objective value of LP \ref{KMZ_LP}. 
\item Our algorithm is \textit{scalable}: we can handle large graphs (up to $\approx 10,000$ vertices), whereas the KMZ algorithm is only practical for graphs with up to $\approx$ 300 vertices due to the bottleneck of solving the (enormous) LP.
\item The large clusters found by our algorithm can be meaningful, in that the algorithm partially discovers ``ground truth" clusters in real-world and synthetic instances. \\
\end{itemize}

Our experiments focus on the exact algorithm. We observe that empirically the exact algorithm is sufficiently fast. 


\paragraph{Real dataset description.} 
We obtained datasets representing social networks from the Stanford Large Network Dataset Collection \cite{FBSocialCircles, feather, HepData}.\footnote{https://snap.stanford.edu/data/ego-Facebook.html} Specifically, we used the \textit{ego-Facebook} dataset containing 10 graphs that are subgraphs of a social network from Facebook. Each subgraph, or \textit{ego-network}, represents a specific user's friend list and the connections within it. We converted this to a complete, signed graph by representing a connection between users as a positive edge, and a non-connection as a negative edge. (See Tables \ref{table: fb_small_statistics} and \ref{table: fb_large_statistics} in Appendix \ref{appendix: add_plots_exp_sec} for statistics on these graphs.) Each ego-network is accompanied by ``ground truth" circles; each circle is a collection of vertices that the user has labelled as a community. We note that the circles are not necessarily partitions of the friend list, as they may overlap or not cover the entire friend list.  

For each Facebook ego-network, we applied our exact algorithm using the matrix multiplication implementation.  For five of the ego-networks that were of small enough size, we also solved the LP in order to bound the approximation ratio of our algorithm.  The LP solver used was Gurobi.  For the latter datasets, we also applied the KMZ algorithm as an additional means of comparison. Let $r_1$ be the radius in $L_t(\cdot)$ and let $r_2$ be the radius used to cut out $C_t$ in Algorithm \ref{KMZ-alg}. While Theorem \ref{thm: apx_thm} holds for $r_1 = 1/5$ and $r_2 = 2/5$, in practice these radii may give an objective value near the maximum positive degree in a sparse graph. We can obtain even better results than those guaranteed by Theorem \ref{thm: apx_thm} by setting the hyperparameters more conservatively. We did parameter sweeps (Figure \ref{fig: sweeps} in Appendix \ref{appendix: add_plots_exp_sec}), and found that $r_1 = r_2 = 0.7$ work well for our algorithm, and $r_1 = r_2 = 0.4$ work well for the KMZ algorithm, so we report the results using these parameters. See also Appendix \ref{appendix: double_parameter_sweep} for the best radii for each dataset. 
Finally, we applied the Pivot algorithm (described in Appendix \ref{appendix: pivot}) to all datasets for an additional comparison \cite{ACN-pivot}. See Tables \ref{table: objectives_fb_small} and \ref{table: objectives_fb_large} and Figure \ref{table: run-times_fb_small}. 

\paragraph{Quality of approximation.} For the five small datasets in Table \ref{table: objectives_fb_small}, the cost of our algorithm is at most 2 times the cost of the LP, and thus at most twice optimal. Our algorithm and the KMZ algorithm performed similarly in terms of objective value. In addition, the fractional cost of the correlation metric and the cost of the LP consistently differ by a factor of around 2. Finally, the objective value of our algorithm is typically slightly less than its fractional cost. For the large data sets (Table \ref{table: objectives_fb_large}) for which it was prohibitive to run the LP, we do not have a lower bound of optimal due to the LP not scaling, so we cannot bound the approximation ratio. For these datasets, we compare to Pivot, which our algorithm outperforms by a substantial margin. 



\begin{center}
\begin{table}[H]
\small
\centering
\begin{tabular}{c | c | c | c | c | c } 
 \hline
  & fractional cost & LP objective & our objective  & KMZ objective  & Pivot objective  \\
\hline
FB 348 & 74.37 & 39.13 & 72 & 89 & 85.03 \\
\hline
FB 414 & 35.53 & 19.66 & 34 & 38 & 50.73 \\
\hline
FB 686 & 58.59 & 30.48 & 47 & 69 & 65.72 \\
\hline
FB 698 & 22.31 & 10.64 & 20 & 18 & 23.51\\
\hline
FB 3980 & 14.31 & 7.34 & 12 & 13 & 16.36 \\
\hline 
\end{tabular}
\captionsetup{width=.9\linewidth}
\caption{Comparison of the fractional values and objective values of our algorithm and the KMZ algorithm for the five small Facebook datasets. The column ``fractional cost" records the fractional cost of the correlation metric. Additionally, we run the Pivot algorithm; the recorded value is the objective value averaged over 500 trials.}
\label{table: objectives_fb_small}
\end{table}
\end{center}



\begin{center}
\begin{table}[H]
\small
\centering
\begin{tabular}{c | c | c | c | c | c } 
 \hline
  & fractional cost & our objective & Pivot objective  & our run-time & \#vertices \\
\hline
FB 0 & 64.02 & 49 & 71.78 & 0.20 & 333\\
\hline
FB 107 & 181.49 & 152 & 216.65 & 1.76 & 1034\\
\hline
FB 1684 & 103.99 & 93 & 130.71 & 0.98 & 786 \\
\hline
FB 1912 & 227.74 & 220 & 259.01 & 0.93 & 747 \\
\hline
FB 3437 & 98.36 & 107 & 99.1 & 0.47 & 534 \\
\hline 
\end{tabular}
\captionsetup{width=.9\linewidth}
\caption{Columns are as in Table \ref{table: objectives_fb_small}. The size of each dataset here makes the LP run-time prohibitive. Run-time is listed in seconds.}
\label{table: objectives_fb_large}
\end{table}
\end{center}

\paragraph{Run-time and scalability.} 
The run-time of our algorithm is significantly faster than that of the KMZ algorithm (Table \ref{table: run-times_fb_small}). For instance, on FB 348, which contains only 224 vertices, the KMZ algorithm took over 30 minutes, whereas our algorithm took a tenth of a second \footnote{Even if we terminate the LP early, e.g., when the primal and dual are within 1 of each other, this still takes at least 10 minutes. Note however that doing so would affect the distances outputted.}. In fact, we can quickly handle very large graphs; on a social network with 12,008 nodes \footnote{https://snap.stanford.edu/data/feather-lastfm-social.html}, our algorithm ran in just over 4 minutes. See Appendix \ref{appendix: scalability} for more details on scalability.  


\paragraph{Comparison to ground truth clusters.} We also analyzed whether the clusters found by our algorithm discovered the ground truth circles identified by users. For each dataset, we considered ``large" clusters of size at least 10, since the small clusters (including several singleton clusters) are less meaningful. For each large cluster, we identified the ground truth circle containing the largest number of vertices from that cluster. The results are plotted in Figure \ref{fig: ground_truth_common_radius} in Appendix \ref{appendix: add_plots_exp_sec}.  We find that for datasets \textsc{FB} 348, 414, 686, 1684, and 1912, almost every large cluster is almost entirely contained in its best ground truth circle (i.e., between 80\% and 100\% of each large cluster is contained in its best ground truth circle). For other datasets, there is less evidence that ground truth circles are being discovered.  




\begin{center}
\begin{table}[H]
\small
\centering
\begin{tabular}{c | c | c | c } 
 \hline
  & our run-time & KMZ run-time & \#vertices \\
\hline
FB 348 & 0.10 & 1847.99 & 224 \\
\hline
FB 414 & 0.06 & 207.92 & 150 \\
\hline
FB 686 & 0.06 & 337.9 & 168 \\
\hline
FB 698 & 0.02 & 3.42 & 61  \\
\hline
FB 3980 & 0.01 & 2.03 & 52 \\
\hline 
\end{tabular}
\captionsetup{width=.9\linewidth}
\caption{A comparison of the run-times (in seconds) of our algorithm and the KMZ algorithm on the five small Facebook datasets.} 
\label{table: run-times_fb_small}
\end{table}
\end{center}



\paragraph{Synthetic datasets.} 
We considered synthetic datasets for two reasons. The first is that running the LP and the KMZ algorithm are prohibitive on many real-world datasets. The second is to further test whether our algorithm discovers ground truth clusters. We took a graph with 100 vertices and 10 positive cliques of size 10 (so the graph admits a perfect clustering) and introduced 20 levels of noise. At each level $i$, we randomly flipped $45i$ edges to the opposite sign. We then applied our algorithm using $r_1 = r_2 = 0.7$ as before. We found that for up to 495 flips ($i=11$), the original clusters of size 10 were almost entirely preserved by our algorithm (in some cases, up to three vertices popped out into singleton clusters). We also found that for all levels of noise we considered, almost every cluster we found was at least 88\% contained in a ground truth cluster (only 6 clusters were an exception to this). See Appendix \ref{appendix: synthetic} for additional plots of these experiments.

==> Correlation Clustering/intro.tex <==
\section{Introduction}


In correlation clustering, a  graph $G= (V,E)$ is given as input, where each edge is labeled either positive $(+)$ or negative $(-)$. If two vertices are connected by a positive edge, this indicates they are similar and want to being clustered together. Alternatively, a negative edge indicates vertices that are dissimilar and want to be in different clusters. 
We make the common assumption that $G$ is complete; that is, there is a labelled edge between each pair of vertices. 

An edge is in \textit{disagreement} with respect to a clustering 
if it is a negative edge and connects two vertices contained inside the same cluster, or if it is a positive edge and connects two vertices in different clusters.
Note that among three or more vertices, 
the positive and negative labels may be such that \textit{any} clustering has some edges in disagreement, e.g. three vertices where the three labels between them are two positives and one negative.

The goal in correlation clustering is to find a clustering that minimizes an objective capturing the edges' disagreements.   
The most widely considered objective is to minimize the $\ell_p$-norm of the disagreements over the vertices. Here, each vertex $u$ has some number, $y(u)$, of disagreements adjacent to it and the goal is to minimize $\sqrt[p]{\sum_{u \in V} y(u)^p}$.  
The most well-studied objective is when $p = 1$, which minimizes the total number of disagreements; the Pivot algorithm is a popular, combinatorial algorithm in this setting \cite{ACN-pivot}.
The case where $p = \infty$ minimizes the maximum number of disagreements at any vertex, which captures a nice notion of fairness in the clustering. 




Our results focus on the $\ell_\infty$-norm objective, which we will refer to as the \textit{Min Max} objective\footnote{Other names for this are the minimax or $\ell_\infty$ objective.}.  
Min Max correlation clustering was first motivated by applications in community detection that are antagonist free,  i.e., there are no members that are largely inconsistent in their community \cite{PM16}. Such problems arise in recommender systems, bioinformatics, and social sciences \cite{cheng2000biclustering, kriegel2009clustering, symeonidis2008nearest, PM16}.

Milenkovic and Puleo \citeyearpar{PM16} initiated the study of Min Max correlation clustering, as well as other $\ell_p$-norms. For all $p \geq 1$, they give a $48$-approximation. Charikar, Gupta, and Schwartz \citeyearpar{CGS17} improved this to a $7$-approximation, and Kalhan, Makarychev, and Zhou \citeyearpar{KMZ19} further improved this to the best known approximation\footnote{Note all of these results are still only for complete graphs.} of 5. 
Milenkovic and Puleo \citeyearpar{PM16} observed that Pivot fails for the $\ell_{\infty}$ norm, even though it gives a 3-approximation in expectation for the $\ell_1$ norm (see the discussion in Appendix A).
See more on correlation clustering in Section~\ref{sec:related}, 
including the interest on fair/local objectives like Min Max.


Previous algorithms on Min Max correlation clustering rounded SDP or LP solutions 
\cite{PM16, CGS17, Khuller2019min, KMZ19}.
The relaxations are large, requiring at least $|V|^3$ constraints and $|V|^2$ variables.  Thus solving them is not practical on even modest sized graphs (e.g. 300-500 vertices). The question looms: does there exist a fast algorithm for Min Max correlation clustering with strong theoretical guarantees?  Moreover, an intriguing direction both towards this question and in its own right is to develop combinatorial algorithms. A key challenge is that it is not clear how to compare to the optimal solution without the LP or SDP, as there are no
non-obvious lower bounds known.


\subsection{Our contributions}

The paper provides fast algorithms for Min Max correlation clustering. 
Our algorithms are the first combinatorial algorithms for the problem with theoretical guarantees.  Our key technical insight that enables these algorithms is the introduction of a semi-metric on the set of vertices, which we call the \textit{\dn}. 
% between pairs of nodes based on their shared positive and negative neighbors. .
The \dn~can be used to set variables in the problem's linear program so that the resulting solution is feasible and provably close to the optimal number of disagreements for the Min Max objective. Thus, we use the LP to compare to the optimal like prior work, but we do not need to solve it since we only use it in the analysis. Our \dn~gives new insights into both correlation clustering and the linear program.  



Let $\omega$ denote the constant for 
the $O(n^{\omega})$ run-time of matrix multiplication on an $n \times n$ matrix, 
where $n = |V|$.  

\begin{theorem} \label{thm: apx_thm}
There is an algorithm that obtains a 40-approximation for Min Max
correlation clustering on complete graphs in time $O(n^{\omega})$.
\end{theorem}

The run-time can be substantially improved when the positive edges of the graph form a sparse graph, which is commonly the case in practice. 

\begin{corollary}\label{cor: apx-sparse}
Suppose all vertices in $V$ have $+$ degree at most $\Delta$,
and for each vertex we are given a list of its positive neighbors.
There is an algorithm that obtains a 40-approximation for 
Min Max correlation clustering on complete graphs in time $O(n \Delta^2 \log n)$.
\end{corollary}
Thus, we have a near-linear time algorithm for sparse graphs.  
This substantially improves on prior work, 
which (to the best of our knowledge) has run-time no better than $O(n^{2 \omega})$ even on sparse graphs
(see Appendix \ref{sec: lp_rounding_alg}).

Next, we show that we can approximate the \dn~to
improve the run-time, even when the graph is dense, 
though at some loss in the approximation factor.  


\begin{theorem} \label{thm: apx_sampling}
Fix $\eps > 0$ sufficiently small.
%, and let $c(\eps)$ be a constant depending only on $\eps$. 
For some constant $c(\eps)$ depending only on $\eps$, there is a randomized algorithm that obtains a $c(\eps)$-approximation for Min Max correlation clustering on complete graphs with probability $1-O(1/n)$ in time $O(n^2\log n/\eps^2)$. 
\end{theorem}


Finally, we show that our theory is predictive of practice (see Section \ref{sec: experiments}). Our algorithm performs similarly in terms of objective value to the algorithm of Kalhan, Makarychev, and Zhou \citeyearpar{KMZ19}, while improving the runtime so substantially that it can feasibly scale to graphs with about 10,000 vertices\footnote{For comparison, the algorithm by Kalhan, Makarychev, and Zhou takes more than 10 minutes on graphs with $\approx$ 200 vertices.}. Moreover, the clusters found by our algorithm are often meaningful in that they partially discover ``ground truth" clusters in real-world and synthetic instances. 






